Dissecting Hessian: Understanding Common Structure of Hessian in Neural Networks

Hessian captures important properties of the deep neural network loss landscape. Previous works have observed low rank structure in the Hessians of neural networks. In this paper, we propose a decoupling conjecture that decomposes the layer-wise Hessians of a network as the Kronecker product of two smaller matrices. We can analyze the properties of these smaller matrices and prove the structure of top eigenspace random 2-layer networks. The decoupling conjecture has several other interesting implications - top eigenspaces for different models have surprisingly high overlap, and top eigenvectors form low rank matrices when they are reshaped into the same shape as the corresponding weight matrix. All of these can be verified empirically for deeper networks. Finally, we use the structure of layer-wise Hessian to get better explicit generalization bounds for neural networks.

==> Misc/acknowledgements.tex <==
We thank ...

==> Misc/contribution.tex <==
Contribution...

==> Old_files/hessian_empirical_old.tex <==
\label{sec:empirical}
We observe several interesting phenomena which can be explained by the structural analysis of Hessian in \cref{sec:hessian}. This shows the Hessians are far from random matrices and Hessians of different models are related. This suggest more meaningful information may be extracted by assessing these common properties. We also further predict and verfy the conditions these phenomenon rely on, and thus provide some connection between network structures and Hessians. 

\subsection{Eigenspace Overlap of different models}
\label{sec:models}
Consider models trained using different random initializations with the same network structure and dataset. We observe surpisingly high top eigenspace overlap between their layerwise Hessians, despite no obvious similarity between their parameters.
%For overparameterized networks, one would expect that they should have very different parameters and thus very different layerwise Hessians. However, we observe that the top eigenspace of their layerwise Hessians have suprisingly high overlap, despite no obvious similarity between their parameters.

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/SubspaceOverlap/LeNet5_fixlr0.01/DimOverlap_CIFAR10_LeNet5_fixlr0.01_conv2.pdf}
        \caption{conv2 ($\xi = 0.027$)}
        \label{fig:Overlap_conv2}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/SubspaceOverlap/LeNet5_fixlr0.01/DimOverlap_CIFAR10_LeNet5_fixlr0.01_fc1.pdf}
        \caption{fc1 ($\xi =0.0047$)}
        \label{fig:Overlap_fc1}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/SubspaceOverlap/LeNet5_fixlr0.01/DimOverlap_CIFAR10_LeNet5_fixlr0.01_fc3.pdf}
        \caption{fc3 ($\xi =0.019$)}
        \label{fig:Overlap_fc3}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspace overlap between models}
    \label{fig:overlap}
\end{figure}

\cref{fig:overlap} shows the pairwise top eigenspace overlap between layerwise Hessians of 6 different models trained on CIFAR-10 with LeNet-5. The overlap is defined as in \cref{eqn:overlap}. We computed the average pairwise overlap (absolute value of normalized dot product) between their parameter vectors ($\xi$ in \cref{fig:overlap}). They are very low and similar to the expectation of random overlap $1/\sqrt{n}$. Also, if this is due to similarity of parameters, we should expect the overlap to stay high instead of having an obvious peak. We also cannot model them as 2 uncorrelated subspace in $\R^d$. In that case, their overlap should be $\frac{k}{d}$ at dimension $k$. Take layer fc1 as an example, the eigenvectors lives in dimension 48000 and are expected to have overlap 0.0025, but the actual overlap is around 0.75 as shown in \cref{fig:Overlap_fc1}.

This phenomenon, however, can be explained using the approximation in \cref{sec:approx_top_eig}. For simplicity, in this subsection we assume exactly $n$ top eigenvectors of layerwise Hessian are in $\Krsp(\tx)$. A more generalized model is in the Appendix.

Now suppose we have 2 different models with $\vt_{\vx1}$ and $\vt_{\vx2}$ respectively. We can approximate their top $k$ eigenspace as $\mU_k \otimes \vt_{\vx1}$ and $\mV_k \otimes \vt_{\vx2}$ respectively, for $k \leq n$. The eigenspace overlap at dimension $k$ is thus
\begin{equation}
\Overlap\left(\mU_k \otimes \vt_{\vx1}, \mV_k \otimes \vt_{\vx2}\right) =\frac{1}{k}\left\|\mV_1^T\mV_2 \otimes \vt_{\vx1}^T\vt_{\vx2}\right\|^2_F= \left(\vt_{\vx1} \cdot \vt_{\vx2}\right)^2\Overlap\left(\mU_k, \mV_k\right).
\label{eqn:model_overlap}
\end{equation}
Moreover, columns of $\mU_k$ and $\mV_k$ lives in $\R^n$, the space corresponding to the neurons. Since output neurons (channels for conv) can be permuted to give equivalent models while changing eigenvectors, we can assume that columns of $\mU_k$ and $\mV_k$ have no correlation and thus have an expected inner product of $\frac{1}{\sqrt{n}}$. Thus, $\Overlap(\mU_k, \mV_k) = \frac{k}{n}$ and the eigenspace overlap of at dimension $k$ would be approximately $\frac{k}{n}(\vt_{\vx1} \cdot \vt_{\vx2})^2$. This explains the peak at dimension $n$ and the linear growth before it. 

Note that fc3 does not have the linear growth since neurons cannot be permuted in the last layer. Also, a high peak means $(\vt_{\vx1} \cdot \vt_{\vx2})$ is large. \ynote{In addition, for the first layer, models with the same dataset would have the same $\tx$, and that would lead to an overlap close to 1 at dimension $n$. Omit since we did not show the first layer}

Then, consider the $(n+1)$th eigenvector of the first model. Since top $n$ eigenvectors span the full space $\Krsp(\vt_{\vx1})$, it will be orthogonal to this space. It will also have low overlap with $\Krsp(\vt_{\vx2})$ since $(\vt_{\vx1} \cdot \vt_{\vx2})$ is large. This explains the immediate drop in eigenspace overlap at dimension $n+1$. \ynote{May not be necessary}

\subsection{Dominating Eigenvectors of Layer-wise Hessian are Low Rank}
The structure of Hessians' eigenvectors is also important for assessing Hessian properties. Let $\vh_i$ be the $i$th eigenvector of a layerwise Hessian. Since it lives in the same space as the weight vector $\vw$ of that layer, we can define an operation $\Mat(\vh_i)$ to reshape $\vh_i$ into a matrix with the same shape as the weight matrix $\mW$. 

The rank of $\Mat(\vh_i)$ can be considered as an indicator of the complexity of the eigenvector. Consider the case that $\vh_i$ is one of the top eigenvectors ($i \leq t$). From \cref{sec:approx_top_eig}, we have $\vh_i \approx \vu_i \otimes \tx$ for some $\vu_i \in \R^n$. Thus, $\Mat(\vh_i) \approx \vu_i\tx^T$ and is approximately rank 1.
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Eigenvec_Lowrank/Top_Eigenvector_rank_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_20_top1_10.pdf}
    \captionsetup{justification=centering}
    \caption{Ratio between spectral norm and Frobenius norm. (LeNet5 on CIFAR10)}
    \label{fig:eigen_lowrank}
\end{figure}

\cref{fig:eigen_lowrank} shows the L2 norm of top $k$ singular values divided by the Frobenius Norm of $\Mat(\vh_i)$, for $k = 1,10$. This value measures how each eigenvector is close to rank $k$. We can see the top few eigenvectors are close to rank 1. This agrees with our prediction. It also shows that the approximation is usually more accurate when $i$ is smaller.

The values are all high for $k=10$ so that all these eigenvectors can be approximated as rank 10 or lower. This results also suggest that eigenvectors of layerwise Hessians have internal structure and cannot be modelled as randomly chosen vectors in a subspace. \ynote{Can be deleted}

\subsection{Outliers in Eigenvalue Spectrum and \texorpdfstring{$\E[\mM]$}{EM}}
\label{sec:emp_outlier}
One characteristic of Hessian that has been mentioned by many is the outliers in the spectrum of eigenvalues. \citet{sagun2017empirical} suggests that there is a gap in Hessian eigenvalue distribution around the number of classes $C$ in most cases, where $C=10$ in our case. \citet{papyan2019measurements} provides further explanation for the $C$ outliers using class clustering. 

Since $\E[\vx\vx^T]$ is close to rank 1 and the Kronecker factorization is a good approximation for top eigenspace, the top eigenvalues of layerwise Hessian can be approximated as the top eigenvalues of $\E[\mM]$ multiplied by the first eigenvalue of $\E[\vx\vx^T]$. Thus, the top eigenvalues of Hessians should have the same relative ratios as the top eigenvalues of their corresponding $\E[\mM]$'s. We can also conjecture that the outliers also appear in $\E[\mM]$.

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/FC2_MNIST/UTAU_vs_full_sigval_d30_MNIST_Exp1_FC2_fixlr0.01R1_E-1_fc1.pdf}
        \caption{FC2 fc1 at minimum\\(MNIST)}
        \label{fig:UTAU_H_spec_FC2}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/LeNet5_fixlr0.01/UTAU_vs_full_sigval_d30_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_fc1.pdf}
        \caption{LeNet5 fc1 at minimum\\(CIFAR10)}
        \label{fig:UTAU_H_spec_Lenet}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/LeNet5_RL/UTAU_vs_full_sigval_d30_CIFAR10_RandomLabel_LeNet5_fixlr0.01_RLR4_E-1_fc1.pdf}
        \caption{LeNet5 fc1 at minimum\\(CIFAR10 Random Label)}
        \label{fig:UTAU_H_spec_RL}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspectrum of $\E[\mM]$ and $\E[\mH]$}
    \label{fig:UTAU_H_spec}
\end{figure}

Figure 7 shows the similarity of eigenvalue spectrum between $\E[\mM]$ and layerwise Hessians in different situations, agreeing with our prediction.

However, the outliers only appear at initialization and at minimum for true labels but not at miminum for random labels, contradicting to the fact that one may assume that random initialization is closer to the case of random labels. 

\citet{papyan2019measurements} provides explanation for the gap in eigenspectrum using class clustering. Although we reproduced their results on their networks, there is no clear class clustering for both $\E[M]$ and layerwise Hessian at the Minimum for networks we experiment on. The reason is unclear but we conjecture that class clustering is only significant for very large networks.

The outliers at initialization, however, are easier to explain. Similar to \citet{papyan2019measurements} suggests for full Hessian, we observe logit clustering in $\E[\mM]$'s. Since there are $C$ logits, we would expect there are $C$ outliers. The results are shown in Appendix.

\subsection{Zero-mean Batch Normalization}
\snote{The approximation worsen, but is still relevant. Reason of low overlap: low correlation between $x$ in different layers, random permutation of neurons in FC layers.}
According to our explanation, the good approximation and high overlap of top eigenspace both depend on the low rank structure of $\E[\vx\vx^T]$. Also, the low rank strcuture is caused by the fact $\E[\vx]\E[\vx]^T]$ dominates $\mSigma_\vx$ in most cases. Thus, we conjecture using Batch normalization (BN) \citep{ioffe2015batch} will change these phenomena as $\E[\vx]$ will be zero and $\E[\vx\vx^T] = \mSigma_\vx$.

We experiment on the same networks but with BN. The results are shown in the Appendix. We found that $\E[\vx\vx^T]$ is no longer close to rank 1 for models trained with BN. However, $\E[\vx\vx^T]$ still have a few large eigenvalues and is not similar to a random matrix.

In the case, our approximation in \cref{sec:approx_top_eig} is not accurate. Thus, the overlap of top $k$ eigenspace between different models can no longer be approximated as in \cref{eqn:model_overlap}. As expected, models with BN give a much lower eigenspace overlap at dimension smaller than $n$ and there is no obvious peak.

The approximation of Hessian eigenvalues using Kronecker factorization is also not so accurate in models using BN, agreeing with our conjecture. However, the approximation still gives meaningful information and the top eigenspace overlap between true and approximated hessian is still (). It is lower than the case without BN but much larger than the expected value for 2 random subspaces.

==> Old_files/hessian_empirical_old_2.tex <==
\label{sec:empirical}
We observe several interesting phenomena which can be explained by the structural analysis of Hessian in \cref{sec:hessian}, demonstrating that the Hessians are far from random matrices and Hessians of different models are related. This observation also suggests that more meaningful information may be extracted by assessing these common properties. We also further predict and verfy the conditions these phenomenon rely on, and thus provide some connection between network structures and Hessians. \znote{Need reorganization, probably some parts can move to conclusion}

\subsection{Eigenspace Overlap of different models}
\label{sec:models}
Consider models trained using different random initializations with the same network structure and dataset. We observe surpisingly high top eigenspace overlap between their layerwise Hessians, despite no obvious similarity between their parameters.
%For overparameterized networks, one would expect that they should have very different parameters and thus very different layerwise Hessians. However, we observe that the top eigenspace of their layerwise Hessians have suprisingly high overlap, despite no obvious similarity between their parameters.

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/SubspaceOverlap/Mix/Overlap_LeNet5_varying_conv2.pdf}
        \caption{conv2-LeNet with 16/25 output channels}
        \label{fig:Overlap_conv2}
    \end{subfigure}%
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/SubspaceOverlap/Mix/Overlap_LeNet5_varying_fc1.pdf}
        \caption{fc1-LeNet5 with 80/100/120/150 output neuron}
        \label{fig:Overlap_fc1}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspace overlap between models\znote{currently working on experiments which have different number of neurons.}}
    \label{fig:overlap}
\end{figure}

\cref{fig:overlap} includes 5 different structural variants of LeNet5 trained on CIFAR-10. For each structural variant, 5 models are trained independently from different random initializations. We plot the average pairwise top eigenspace overlap between layerwise Hessians among those 5 models.\znote{Not sure if this explanation is clear enough.} For example, in \cref{fig:Overlap_conv2} we consider the vanilla LeNet5, whose conv2 layer has $n=16$ output channels, and a modified LeNet5, whose conv2 has $n=25$ output channels. It is clear that for the same structure, the top eigenspaces of different models exhibits a highly non-trivial overlap, and the overlap peaks near $n$, which is the dimension of the layer's output. For sanity check, pairwise dot product between the weight matrices of different models are computed, and there does not appear to be notable correlation.


%We computed the average pairwise overlap (absolute value of normalized dot product) between their parameter vectors ($\xi$ in \cref{fig:overlap}). They are very low and similar to the expectation of random overlap $1/\sqrt{n}$. Also, if this is due to similarity of parameters, we should expect the overlap to stay high instead of having an obvious peak. We also cannot model them as 2 uncorrelated subspace in $\R^d$. In that case, their overlap should be $\frac{k}{d}$ at dimension $k$. Take layer fc1 as an example, the eigenvectors lives in dimension 48000 and are expected to have overlap 0.0025, but the actual overlap is around 0.75 as shown in \cref{fig:Overlap_fc1}.

This phenomenon can be explained using the approximation in \cref{sec:approx_top_eig}. For simplicity, in this subsection we assume exactly $n$ top eigenvectors of layerwise Hessian are in $\Krsp(\hE[\vx])$. A more generalized model is in the Appendix.

Now suppose we have 2 different models with $\hE[\vx]_1$ and $\hE[\vx]_2$ respectively. We can approximate their top $k$ eigenspace as $\mU_k \otimes \hE[\vx]_1$ and $\mV_k \otimes \hE[\vx]_2$ respectively, for $k \leq n$. The eigenspace overlap at dimension $k$ is thus
\begin{equation}
\begin{aligned}
    \Overlap\left(\mU_k \otimes \hE[\vx]_1, \mV_k \otimes \hE[\vx]_2\right) &=\frac{1}{k}\left\|\mV_1^T\mV_2 \otimes \hE[\vx]_1^T\hE[\vx]_2\right\|^2_F\\
    &= \left(\hE[\vx]_1 \cdot \hE[\vx]_2\right)^2\Overlap\left(\mU_k, \mV_k\right).
\end{aligned}
\label{eqn:model_overlap}
\end{equation}
Moreover, columns of $\mU_k$ and $\mV_k$ lives in $\R^n$, the space corresponding to the neurons. Since output neurons (channels for conv) can be permuted to give equivalent models while changing eigenvectors, we can assume that columns of $\mU_k$ and $\mV_k$ have no correlation and thus have an expected inner product of $\frac{1}{\sqrt{n}}$. Thus, $\Overlap(\mU_k, \mV_k) = \frac{k}{n}$ and the eigenspace overlap of at dimension $k$ would be approximately $\frac{k}{n}(\hE[\vx]_1 \cdot \hE[\vx]_2)^2$. This explains the peak at dimension $n$ and the linear growth before it. 

When $k=n$, the overlap is approximately $\hE[\vx]_1 \cdot \hE[\vx]_2$. Since $\hE[\vx]_1$ and $\hE[\vx]_2$ are the same for the input layer and all non-negative for other layers, the overlap is expected to be high at dimension $n$. \ynote{One problem for this statement is the overlap is not very close to 1 for the input layer. Probably we can also explain by saying our explanation is not very accurate.}

Note that fc3 does not have the linear growth since neurons cannot be permuted in the last layer. \ynote{In addition, for the first layer, models with the same dataset would have the same $\hE[\vx]$, and that would lead to an overlap close to 1 at dimension $n$. Omit since we did not show the first layer}

Then, consider the $(n+1)$th eigenvector of the first model. Since top $n$ eigenvectors span the full space $\Krsp(\hE[\vx]_1)$, it will be orthogonal to this space. It will also have low overlap with $\Krsp(\hE[\vx]_2)$ since $(\hE[\vx]_1 \cdot \hE[\vx]_2)$ is large. This explains the immediate drop in eigenspace overlap at dimension $n+1$. \ynote{May not be necessary}

\subsection{Dominating Eigenvectors of Layer-wise Hessian are Low Rank}
\label{sec:domin_eig}
The structure of Hessians' eigenvectors is also important for assessing Hessian properties. Let $\vh_i$ be the $i$th eigenvector of a layerwise Hessian. Since it lives in the same space as the weight vector $\vw$ of that layer, we can define an operation $\Mat(\vh_i)$ to reshape $\vh_i$ into a matrix with the same shape as the weight matrix $\mW$. \ynote{The definition of $\Mat$ can be removed if we define it in Section 3 or 4}

The rank of $\Mat(\vh_i)$ can be considered as an indicator of the complexity of the eigenvector. Consider the case that $\vh_i$ is one of the top eigenvectors ($i \leq t$). From \cref{sec:approx_top_eig}, we have $\vh_i \approx \vu_i \otimes \hE[\vx]$ for some $\vu_i \in \R^n$. Thus, $\Mat(\vh_i) \approx \vu_i\hE[\vx]^T$ and is approximately rank 1.
\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Eigenvec_Lowrank/NLeNet_base/Top_Eigenvector_rank_CIFAR10_Exp1_LeNet5_normnew_fixlr0.01R1_E-1_20.pdf}
    \captionsetup{justification=centering}
    \caption{Ratio between top singular value and Frobenius norm. (LeNet5 on CIFAR10)}
    \label{fig:eigen_lowrank}
\end{figure}

\cref{fig:eigen_lowrank} shows the L2 norm of top $k$ singular values divided by the Frobenius Norm of $\Mat(\vh_i)$, for $k = 1$. This value measures how each eigenvector is close to rank $k$. We can see the top few eigenvectors are close to rank 1. This agrees with our prediction. It also shows that the approximation is usually more accurate when $i$ is smaller.

% The values are all high for $k=10$ so that all these eigenvectors can be approximated as rank 10 or lower. This results also suggest that eigenvectors of layerwise Hessians have internal structure and cannot be modelled as randomly chosen vectors in a subspace. \ynote{Can be deleted}

\subsection{Outliers in Eigenvalue Spectrum and \texorpdfstring{$\E[\mM]$}{EM}}
\label{sec:emp_outlier}
One characteristic of Hessian that has been mentioned by many is the outliers in the spectrum of eigenvalues. \citet{sagun2017empirical} suggests that there is a gap in Hessian eigenvalue distribution around the number of classes $C$ in most cases, where $C=10$ in our case. \citet{papyan2019measurements} attempted further explanation for the $C$ outliers using class clustering. 

Since $\E[\vx\vx^T]$ is close to rank 1 and the Kronecker factorization is a good approximation for top eigenspace, the top eigenvalues of layerwise Hessian can be approximated as the top eigenvalues of $\E[\mM]$ multiplied by the first eigenvalue of $\E[\vx\vx^T]$. Thus, the top eigenvalues of Hessians should have the same relative ratios as the top eigenvalues of their corresponding $\E[\mM]$'s. We can also conjecture that the outliers also appear in $\E[\mM]$.

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/FC2_MNIST/UTAU_vs_full_sigval_d30_MNIST_Exp1_FC2_fixlr0.01R1_E-1_fc1.pdf}
        \caption{FC2 fc1 at minimum\\(MNIST)}
        \label{fig:UTAU_H_spec_FC2}
    \end{subfigure}%
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/LeNet5_fixlr0.01/UTAU_vs_full_sigval_d30_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_fc1.pdf}
        \caption{LeNet5 fc1 at minimum\\(CIFAR10)}
        \label{fig:UTAU_H_spec_Lenet}
    \end{subfigure}%
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/EM_vs_H/LeNet5_RL/UTAU_vs_full_sigval_d30_CIFAR10_RandomLabel_LeNet5_fixlr0.01_RLR4_E-1_fc1.pdf}
        \caption{LeNet5 fc1 at minimum\\(CIFAR10 Random Label)}
        \label{fig:UTAU_H_spec_RL}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspectrum of $\E[\mM]$ and $\E[\mH]$}
    \label{fig:UTAU_H_spec}
\end{figure}

Figure 7 shows the similarity of eigenvalue spectrum between $\E[\mM]$ and layerwise Hessians in different situations, agreeing with our prediction. However, the outliers only appear at initialization and at minimum for true labels but not at miminum for random labels.

\citet{papyan2019measurements} provides explanation for the gap in eigenspectrum using class clustering. Although we reproduced their results on their networks, there is no clear class clustering for both $\E[M]$ and layerwise Hessian at the Minimum for networks we experiment on. The reason is unclear but we conjecture that class clustering is only significant for very large networks.

The outliers at initialization, however, are easier to explain. Similar to \citet{papyan2019measurements} suggests for full Hessian, we observe logit clustering in $\E[\mM]$'s. Since there are $C$ logits, we would expect there are $C$ outliers. The results are shown in Appendix.

\subsection{Zero-mean Input and Batch Normalization}
\snote{The approximation worsen, but is still relevant. Reason of low overlap: low correlation between $x$ in different layers, random permutation of neurons in FC layers.}
According to our explanation, the good approximation and high overlap of top eigenspace both depend on the low rank structure of $\E[\vx\vx^T]$. Also, the low rank strcuture is caused by the fact $\E[\vx]\E[\vx]^T]$ dominates $\mSigma_\vx$ in most cases. Thus, we conjecture using Batch normalization (BN) \citep{ioffe2015batch} will change these phenomena as $\E[\vx]$ will be zero and $\E[\vx\vx^T] = \mSigma_\vx$.

We experiment on the same networks but with BN. The results are shown in the Appendix. We found that $\E[\vx\vx^T]$ is no longer close to rank 1 for models trained with BN. However, $\E[\vx\vx^T]$ still have a few large eigenvalues and is not similar to a random matrix.

In the case, our approximation in \cref{sec:approx_top_eig} is not accurate. Thus, the overlap of top $k$ eigenspace between different models can no longer be approximated as in \cref{eqn:model_overlap}. As expected, models with BN give a much lower eigenspace overlap at dimension smaller than $n$ and there is no obvious peak.

The approximation of Hessian eigenvalues using Kronecker factorization is also not so accurate in models using BN, agreeing with our conjecture. However, the approximation still gives meaningful information and the top eigenspace overlap between true and approximated hessian is still (). It is lower than the case without BN but much larger than the expected value for 2 random subspaces.

==> Old_files/hessian_structure_old.tex <==
\label{sec:hessian}

\rnote{Title of this section is a bit long and don't have a real focus. We might consider break it into multiple sections? One possibility is that we talk about the decomposition, then talk about properties of $xx^T$ (both zero-mean and non-zero-mean case) and briefly talk about properties of $M$ (mostly empirical); in the next section we can then use this decomposition to justify (a) Hessian overlap; (b) low rank structure of the top eigenvectors; (c) rank C-1 Hessian}

The fact that layer-wise Hessian for fully connected layers can be decomposed into the expectation of Kronecker products as in \cref{eqn:decomp} poses a natural question: Can the Hessian be approximated using the Kronecker product of the expectations? That is, whether 
\begin{equation}
    \HessL^{(p)}(\theta) = \E\left[\mM\otimes \vx\vx^T\right] \approx \E[\mM] \otimes \E[\vx\vx^T]. 
\end{equation}

\rnote{Maybe we should call the above a conjecture with a name (something like ``the decoupling conjecture''?), then we say that empirically we show the conjecture is true, and this has a lot of benefits.}

If yes, we can analyze the layer-wise Hessian by analyzing of the two components. Note that $\E[\mM]$ is the Hessian of the layer-wise output with respect to empirical loss, and $\E[\vx\vx^T]$ is the auto-correlation matrix of the layer-wise inputs. For simplicity we call $\E[\mM]$ the output Hessian and $\E[\vx\vx^T]$ the input auto-correlation. 

Moreover, we can approximate the eigenvectors and eigenvalues of the layer-wise Hessian $\HessL^{(p)}(\theta)$ by $\E[\mM]$ and $\E[\vx\vx^T]$. Let $\vm$ and $\vv$ be an eigenvector of $\E[\mM]$ and $\E[\vx\vx^T]$ respectively, with corresponding eigenvalues $\lambda_\vm$ and $\lambda_\vv$. Since both matrices are positive semi-definite, $\vm \otimes \vv$ is an eigenvector of $\E[\mM] \otimes \E[\vx\vx^T]$ with eigenvalue $\lambda_\vm\lambda_\vv$. In this way, since $\E[\mM]$ has $n$ eigenvectors and $\E[\vx\vx^T]$ has $m$ eigenvectors, we can approximate all $mn$ eigenvectors for the layerwise Hessian.

As both $\E[\mM]$ and $\E[\vx\vx^T]$ can be computed in time comparable to back-propagation, algorithm then provides us with a fast inference of second order information. Also, explicit calculation of the layerwise Hessian requires $O(m^2n^2)$ space but our approximation only requires $O(m^2+n^2)$ space. 

Similar approximation for Fisher Information matrices have been used in K-FAC optimization algorithm \citep{martens2015optimizing}. While they gives efficient calculation for the matrix inverse, our analysis focuses more on the structure analysis. Also, unlike Fisher Information matrices, we can calculate top eigenvalues and eigenvectors of the Hessian efficiently \citep{yao2019pyhessian} so that the approximation of top eigenspace can be directly compared. \ynote{Put in for comparison, maybe unnecessary}

For convolutional layers (convs), we proposed a similar Kronecker factorization motivated by \citet{grosse2016kronecker}. We also denote it as $\E[\mM]\otimes \E[\vx\vx^T]$, with a different definition of $\mM$.(See \cref{sec:appendix_conv} for details) \ynote{Where should we put this paragraph?}.
\subsection{Hessian Approximation}
We run experiments on both CIFAR-10 and MNIST \cnote{May need to cite these datasets} using several different Fully Connected (FC) networks and LeNets, where we only analyze the FC layers\cnote{Not sure whether want to emphasize this}. All the experiments give qualitatively similar results. The results shown are for networks .... Other results are shown in the Appendix. The exact eigenvalues and eigenvectors of the layer-wise Hessians are computed using a modified Lanczos algorithm\znote{need description in appendix on the modified Lanczos.}

Empirical results show that this approximation works reasonably well, especially for the top eigenvalues and eigenspace, as shown in \cref{fig:approx_result} The eigenvectors are ranked in the order of decreasing eigenvalues. The overlap at dimension $k$ is the overlap of subspaces consist of top $k$ eigenvectors. We define the subspace overlap as the L2 average of the cosine of canonical angles: For $k$-dimensional subspaces $\mU,\mV$ in $\R^d$ ($d\geq k$) where the basis vectors $\vu_i$s and $\vv_i$s are column vectors, we define the subspace overlap of $\mU$ and $\mV$ as
\begin{equation}
    \Overlap(\mU, \mV) := \frac{1}{k}\|\mU^T\mV\|^2_F =\frac{1}{k}\|\cos\vtheta\|^2,
    \label{eqn:overlap}
\end{equation}
where $\vtheta$ is the size $k$ vector of canonical angles between $\mU$ and $\mV$. It is equivalent to the definition in \citet{gur2018gradient}.(Proof shown in appendix)

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/ApproxQuality/FC2_fixlr/sample_kron_decomp_traceoverlap_d80_MNIST_Exp1_FC2_fixlr0.01R2_E-1.pdf}
        \caption{Subspace overlap between\\ approximated and exact layer-wise hessian}
        \label{fig:overlap_approx}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.495\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/ApproxQuality/FC2_fixlr/eigenval_compare_top50_MNIST_Exp1_FC2_fixlr0.01R2_E-1_fc2.pdf}
        \caption{Top eigenvalues of approximated\\ and exact layer-wise hessian\cnote{Need to specify which layer it is.}}
        \label{fig:eigenval_approx}
    \end{subfigure}
    \caption{FC2 MNIST \znote{To be completed}}
    \label{fig:approx_result}
\end{figure}

\subsection{Eigenvector Correspondence}
\label{sec:eigen_corr}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/xxT_Trueest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{$\E[\vx\vx^T]$}
        \label{fig:Corr_xxT_True_fc}
    \end{subfigure}
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/UTAU_Trueest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{$\E[\mM]$}
        \label{fig:Corr_UTAU_True_fc}
    \end{subfigure}
    \begin{subfigure}[t]{0.065\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/Misc/colorbar.pdf}
    \end{subfigure}
    \caption{Eigenvector Correspondence for fc1 in LeNet5 ($n$=120)}
    \label{fig:Corr_fc}
\end{figure}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/Conv/xxT_Trueest_real_corr_expand_t50_CIFAR10_Exp1_LeNet5_fixlr0.01_E-1_conv2.pdf}
        \caption{$\E[\vx\vx^T]$}
        \label{fig:Corr_xxT_True_conv}
    \end{subfigure}
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/Conv/UTAU_Trueest_real_corr_expand_t50_CIFAR10_Exp1_LeNet5_fixlr0.01_E-1_conv2.pdf}
        \caption{$\E[\mM]$}
        \label{fig:Corr_UTAU_True_conv}
    \end{subfigure}
    \begin{subfigure}[t]{0.04\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/Misc/colorbar.pdf}
    \end{subfigure}
    \caption{Eigenvector Correspondence for conv2 in LeNet5 ($n$=16)}
    \label{fig:Corr_conv}
\end{figure}
To better visualize how eigenvectors of layer-wise Hessian are correlated with eigenvectors of $\E[\mM]$ and $\E[\vx\vx^T]$, we introduce `eigenvector correspondence matrices' as shown in \cref{fig:Corr_fc} and \cref{fig:Corr_conv}. Take $\E[\vx\vx^T]$ as an example. Let $\vv_i$ be the $i$th eigenvector of $\E[\vx\vx^T]$ and $\vh_j$ be the $j$th eigenvector of layer-wise Hessian, both ranking in decreasing order of eigenvalues. We can then define $\Krsp(\vv_i)$ as the $n$\cnote{What is $n$?} dimensional subspace of $\vv_i$'s Kronecker products\cnote{It's still confusing to me if you say ``one's Kronecker products'' because Kronecker product is a binary operator, perhaps use ``one's Kronecker products with xxx'' instead?} in $\R^{mn}$ where $\vh_j$ lives in\cnote{What's Krsp? Is it defined in the next sentence?}. Columns of $\mI_n \otimes \vv_i$ form the basis for $\Krsp(\vv_i)$. We can then define the correspondence between $\vv_i$ and $\vh_j$ as
\begin{equation}
    \Corr(\vv_i, \vh_j) = \|(\mI_n \otimes \vv_i)^T\vh_j\|^2.
\end{equation}
Its value is shown in the $(i,j)$-entry of the heatmap. The eigenvector correspondence for $\E[\mM]$ is defined in the same way, except that the subspace for $\E[\mM]$'s $i$th eigenvector $\vm_i$ is $\vm_i \otimes \mI_m$.
\cnote{I think this subsection is very hard for the readers to understand. My suggestion is to interpret our result in a reverse way, i.e., we first hypothesize that our approximation is totally accurate, then the top eigenvectors of Hessian should be the top eigenvector of $E[xx^T]$ Kronecker with the top eigenvectors of $E[M]$, and we design this method to test our hypothesis, and then show the figures. Besides, for the figures, I think we need more interpretations instead of letting the readers look at them directly. We can perhaps say ``We can see a diagonal pattern in Figure x, indicating that the $i$-th eigenvector of the layerwise Hessian indeed mainly comes from xxx''.}

\subsection{Further Approximation for the Top Eigenspace of Layerwise Hessian}
\label{sec:approx_top_eig}
If $\Corr(\vv_i, \vh_j) \approx 1$, we have $\vh_j \approx \vu \otimes \vv_i$, with some $\vu \in \R^n$. We can also say $\vh_j \in \Krsp(\vv_i)$. We define the first eigenvector of $\E[\vx\vx^T]$ as $\tx$. In both \cref{fig:Corr_fc} and \cref{fig:Corr_conv}, around $n$ top eigenvectors of layer-wise Hessian are all in $\Krsp(\tx)$.

Let the number of top eigenvectors of layerwise Hessian are approximated in $\Krsp(\tx)$ be $s$. In most cases as in \cref{fig:Corr_fc} and \cref{fig:Corr_conv}, $s \approx n$. Thus, for $i \leq s$, $i$th eigenvector $\vh_i \approx \vu_i \otimes \hE[\vx]$ for some $\vu_i \in \R^n$. Thus, for any $k \leq s$, the top $k$ eigenspace of the Hessian can be approximated as $\mU_k \otimes \hE[\vx]$, where columns of $\mU_k$ are $\vu_1, \ldots, \vu_k$.

\cnote{I fell like we are using too many formulas and a bit complicated notations, which will confuse the readers. Here perhaps we need to remind people what is Krsp and what is n. I think it's better to interpret things by words instead of formulas in the main text since this is not really a theoretical paper. For example, for the last sentence in the above paragraph, we can instead say ``Thus, the top $s$ eigenvectors of the Hessian can be well approximated by the Kronecker products between $E[x]$ and the top eigenvectors of $E[M]$.'' I would assume that people can only remember what is $M$ and $xx^T$, so perhaps we need to avoid using notations like $u_i$ if possible. Also, I think the use of ``temporary variables'' is not necessary in most of the texts. We can use English instead, and it also saves some space I guess. I mean, instead of saying ``$\forall i\leq s$'', we can say ``for the first $s$ eigenvectors of ...''}

Also, for some FC layers, the eigenvector correspondance heatmap of $\E[\mM]$ has a diagonal pattern in the first $s$ columns, as shown in \cref{fig:Corr_fc}. We can further approximate the $\vu_i$'s as the $i$th eigenvector of $\E[\mM]$. In this case, $\mU_k$ is the top $k$ eigenspace of $\E[\mM]$. There are also some cases where $s$ is considerably smaller than $n$, and larger than $n$ in rare cases. We will discuss them in the Appendix.
\subsection{Structure of Auto-correlation Matrix \texorpdfstring{$\E[\vx\vx^T]$}{ExxT}}
\label{sec:xxT}
The importance of the first eigenvector of $\E[\vx\vx^T]$, $\tx$, leads us to the analyze the structure of $\E[\vx\vx^T]$. From \cref{fig:xxT}, we can see $\E[\vx\vx^T]$ are all close to rank 1. This phenomenon is also observed along the training trajectory and in other networks.
\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxT_sigval_d20_MNIST_Exp1_FC2_fixlr0.01R1_E-1_fc1fc2.pdf}
        \caption{Fully connected layers of FC2 (MNIST)}
        \label{fig:xxT_sig_fc2}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxT_sigval_d20_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_fc1fc2.pdf}
        \caption{Fully connected layers of LeNet5 (CIFAR10)}
        \label{fig:xxT_sig_lenet}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxTConv_sigval_d20_CIFAR10_Exp1_LeNet5_fixlr0.01_E-1.pdf}
        \caption{Convolution layers of LeNet5 (CIFAR10)}
        \label{fig:xxT_sig_lenet}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspectrum of $\E[\vx\vx^T]$ for different layers in different models. All are close to rank 1.}
    \label{fig:xxT}
\end{figure}

Let the $\hE[\vx]$ be normalized $\E[\vx]$ (first left singular vector of $\E[\vx]$ for conv). We also find that $\tx$ is almost equal to $\hE[\vx]$ (or the top singular vector of $\hE[x]$ for conv), as their inner product are usually larger than 0.998, except for the input layer where the input is close to zero-mean. This suggests that $\E[\vx]\E[\vx]^T$ approximately equals to $\E[\vx\vx^T]$ and dominates the covariance $\mSigma_\vx$. It is verified as the Spectral norm of $\E[\vx]\E[\vx]^T$ is more than 5 times that of $\mSigma_\vx$ in all our experiments. This is natural because $\vx$ are output of ReLU layers and thus nonnegative, for all layers other than the input layer.
 \rnote{We should just show the empirical observation that the covariance matrix has small spectral norm, therefore by standard matrix perturbation bounds the true matrix is still close to rank 1 and the top eigenvector is close to $\E[x]$}


==> Old_files/hessian_structure_old_2.tex <==
\label{sec:hessian}

%\rnote{Title of this section is a bit long and don't have a real focus. We might consider break it into multiple sections? One possibility is that we talk about the decomposition, then talk about properties of $xx^T$ (both zero-mean and non-zero-mean case) and briefly talk about properties of $M$ (mostly empirical); in the next section we can then use this decomposition to justify (a) Hessian overlap; (b) low rank structure of the top eigenvectors; (c) rank C-1 Hessian}

The fact that layer-wise Hessian for fully connected layers can be decomposed into the expectation of Kronecker products as in \cref{eqn:decomp} poses a natural question: Can the Hessian be approximated using the Kronecker product of the expectations? That is, whether 
\begin{equation}
    \HessL^{(p)}(\theta) = \E\left[\mM\otimes \vx\vx^T\right] \approx \E[\mM] \otimes \E[\vx\vx^T]. 
\end{equation}

We call the above conjecture ``the decoupling conjecture''. Equivalently, we conjecture that the two matrices $\mM$ and $\vx\vx^T$ are approximately statistically independent.

%\rnote{Maybe we should call the above a conjecture with a name (something like ``the decoupling conjecture''?), then we say that empirically we show the conjecture is true, and this has a lot of benefits.}

If this conjecture is true, we can analyze the layer-wise Hessian by analyzing the two components separately. Note that $\E[\mM]$ is the Hessian of the layer-wise output with respect to empirical loss, and $\E[\vx\vx^T]$ is the auto-correlation matrix of the layer-wise inputs. For simplicity we call $\E[\mM]$ the output Hessian and $\E[\vx\vx^T]$ the input auto-correlation.

As both $\E[\mM]$ and $\E[\vx\vx^T]$ can be computed in time comparable to back-propagation, algorithm then provides us with a fast inference of second order information. Also, explicit calculation of the layerwise Hessian requires $O(m^2n^2)$ space but our approximation only requires $O(m^2+n^2)$ space.

Moreover, we can approximate the eigenvectors and eigenvalues of the layer-wise Hessian $\HessL^{(p)}(\theta)$ by $\E[\mM]$ and $\E[\vx\vx^T]$. Let $\vm$ and $\vv$ be an eigenvector of $\E[\mM]$ and $\E[\vx\vx^T]$ respectively, with corresponding eigenvalues $\lambda_\vm$ and $\lambda_\vv$. Since both matrices are positive semi-definite, $\vm \otimes \vv$ is an eigenvector of $\E[\mM] \otimes \E[\vx\vx^T]$ with eigenvalue $\lambda_\vm\lambda_\vv$. In this way, since $\E[\mM]$ has $n$ eigenvectors and $\E[\vx\vx^T]$ has $m$ eigenvectors, we can approximate all $mn$ eigenvectors for the layerwise Hessian.

Similar approximation for Fisher Information matrices have been used in K-FAC \citep{martens2015optimizing}. While they give efficient calculation for the matrix inverse, our analysis focuses more on the structural analysis. Besides, unlike K-FAC, we can calculate top eigenvalues and eigenvectors of the Hessian efficiently \citep{yao2019pyhessian} so that the approximation of top eigenspace can be directly compared. \ynote{Put in for comparison, can be deleted}

For convolutional layers (convs), we propose a similar Kronecker factorization motivated by \citet{grosse2016kronecker}. We also denote it as $\E[\mM]\otimes \E[\vx\vx^T]$ but with a different definition of $\mM$.(See \cref{sec:appendix_conv} for details) \ynote{Where should we put this paragraph?}\cnote{I think it's ok to put it here.}
\subsection{Hessian Approximation}
We conduct experiment on CIFAR-10 \citep{Krizhevsky09learningmultiple} and MNIST \citep{lecun1998gradient} dataset using several different Fully Connected (FC) networks, several variations of LeNet \citep{lecun1998gradient}, and VGG11 \citep{simonyan2014very}. The results shown in the main text are variants of LeNet5 trained on CIFAR-10 and FC2 trained on MNIST. Other representative results are shown in \cref{sec:appendix_exp_res}. The eigenvalues and eigenvectors of the exact layer-wise Hessians are approximated using a modified Lanczos algorithm, which is described in detail in \cref{sec:appendix_eigencomp}.

To verify the validity of the approximation, we compare the eigenvalues and top eigenspaces of the approximated Hessian and the true Hessian.
We define the dimension $k$ top eigenspace of a matrix as the subspace spanned by the eigenvectors corresponding to its $k$ largest eigenvalues.

\theoremstyle{definition}
\begin{definition}[Subspace Overlap]
For $k$-dimensional subspaces $\mU,\mV$ in $\R^d$ ($d\geq k$) where the basis vectors $\vu_i$s and $\vv_i$s are column vectors, with $\vtheta$ as the size $k$ vector of canonical angles between $\mU$ and $\mV$, we define the subspace overlap of $\mU$ and $\mV$ as
\begin{equation}
    \Overlap(\mU, \mV) := \frac{1}{k}\|\mU^T\mV\|^2_F =\frac{1}{k}\|\cos\vtheta\|^2.
    \label{eqn:overlap}
\end{equation}
\end{definition}

For two $k$-dimensional subspaces in the same space,
we define the subspace overlap as the L2 average of the cosine of canonical angles: For $k$-dimensional subspaces $\mU,\mV$ in $\R^d$ ($d\geq k$) where the basis vectors $\vu_i$s and $\vv_i$s are column vectors. . we define the subspace overlap of $\mU$ and $\mV$ as
\begin{equation}
    \Overlap(\mU, \mV) := \frac{1}{k}\|\mU^T\mV\|^2_F =\frac{1}{k}\|\cos\vtheta\|^2,
    \label{eqn:overlap}
\end{equation}
Note that when $k=1$, the overlap is equivalent to the dot between the two vectors. This definition is equivalent to the definition in \citet{gur2018gradient}.(Proof shown in appendix\cnote{Remember to specify which part of appendix})

Empirical results show that this approximation works reasonably well, especially for the top eigenvalues and eigenspace, as shown in \cref{fig:approx_result}. The eigenvectors are ranked in the order of decreasing eigenvalues, and the overlap at dimension $k$ is the overlap of subspaces consist of top $k$ eigenvectors. 

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/ApproxQuality/FC2_fixlr/sample_kron_decomp_traceoverlap_d80_MNIST_Exp1_FC2_fixlr0.01R2_E-1.pdf}
        \caption{Subspace overlap between\\ approximated and exact layer-wise hessian}
        \label{fig:overlap_approx}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/ApproxQuality/FC2_fixlr/eigenval_compare_top50_MNIST_Exp1_FC2_fixlr0.01R2_E-1_fc2.pdf}
        \caption{Top eigenvalues of approximated\\ and exact layer-wise Hessian for fc2-FC2}
        \label{fig:eigenval_approx}
    \end{subfigure}
    \caption{FC2 MNIST \znote{To be completed}}
    \label{fig:approx_result}
\end{figure}
\subsection{Eigenvector Correspondence}
\label{sec:eigen_corr}
\begin{figure}[ht]
    \centering
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/xxT_Trueest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{True Hessian with $\E[\vx\vx^T]$}
        \label{fig:Corr_xxT_True_fc}
    \end{subfigure}%
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/UTAU_Trueest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{True Hessian with $\E[\mM]$}
        \label{fig:Corr_UTAU_True_fc}
    \end{subfigure}%
    \begin{subfigure}[t]{0.065\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/Misc/colorbar.pdf}
    \end{subfigure}
    \bigskip
\begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/xxT_Approxest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{Approximated Hessian with $\E[\vx\vx^T]$}
        \label{fig:Corr_xxT_Approx_fc}
    \end{subfigure}%
    \begin{subfigure}[t]{0.46\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Correspondence/LeNet5_fixlr0.01/UTAU_Approxest_real_corr_expand_t200_CIFAR10_Exp1_LeNet5_fixlr0.01R2_E-1_fc1.pdf}
        \caption{Approximated Hessian with $\E[\vx\vx^T]$}
        \label{fig:Corr_UTAU_Approx_fc}
    \end{subfigure}%
    \begin{subfigure}[t]{0.065\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/Misc/colorbar.pdf}
    \end{subfigure}
    \caption{Eigenvector Correspondence for fc1 in LeNet5 ($n$=120)}
    \label{fig:Corr_fc_approx}
\end{figure}
To better visualize how eigenvectors of layer-wise Hessian are correlated with eigenvectors of $\E[\mM]$ and $\E[\vx\vx^T]$, we introduce `eigenvector correspondence matrices' as shown in \cref{fig:Corr_fc_approx}. Take $\E[\vx\vx^T]$ as an example. Let $\vv_i$ be the $i$th eigenvector of $\E[\vx\vx^T]$ and $\vh_j$ be the $j$th eigenvector of layer-wise Hessian, both ranking in decreasing order of eigenvalues. We can then define $\Krsp(\vv_i)$ as the $n$ dimensional subspace of $\vv_i$'s Kronecker products in $\R^{mn}$ where $\vh_j$ lives in.\cnote{It's still confusing to me if you say ``one's Kronecker products'' because Kronecker product is a binary operator, perhaps use ``one's Kronecker products with xxx'' instead?} Columns of $\mI_n \otimes \vv_i$ form the basis for $\Krsp(\vv_i)$. 
Since $\vh_j$ lives in the same space as the weight vector $\vw$ of that layer, we can define an operation $\Mat(\vh_i)$ to reshape $\vh_i$ into a matrix with the same shape as the weight matrix $\mW$. \ynote{Should we move this defintion of $\Mat$ to Section 3? Also we can choose one version of explanation between the subspace of Kronecker products and the reshape into the shape of weight matrix, but this may require a rephrase of all the explanations below in Seciton 4.}
\znote{Do we include this in a definition environment}

We can then define the correspondence between $\vv_i$ and $\vh_j$ as
\begin{equation}
    \Corr(\vv_i, \vh_j) = \|(\mI_n \otimes \vv_i)^T\vh_j\|^2 = \|\Mat(\vh_j)\vv_i\|^2,
\end{equation}
where 
Its value is shown in the $(i,j)$-entry of the heatmap. The eigenvector correspondence for $\E[\mM]$ is defined in the same way, except that the subspace for $\E[\mM]$'s $i$th eigenvector $\vm_i$ is $\vm_i \otimes \mI_m$. (Or $\|\Mat(\vh_j)^T\vm_i\|^2$ if we use the second definition.)

If $\Corr(\vv_i, \vh_j) \approx 1$, we have $\vh_j \approx \vu \otimes \vv_i$, with some $\vu \in \R^n$. \ynote{Or state $\Mat(\vh_j)^T = \vu\vv_i^T$, we can then omit this in \cref{sec:domin_eig} }We can also say $\vh_j \in \Krsp(\vv_i)$. From \cref{fig:Corr_fc} and \cref{fig:Corr_conv}, we can see that around $n$ top eigenvectors are in $\Krsp(\vv_1)$, where $\vv_1$ is the first eigenvector of $\E[\vx\vx^T]$. This leads us to analyze the structure of $\E[\vx\vx^T]$.
\cnote{I think this subsection is very hard for the readers to understand. My suggestion is to interpret our result in a reverse way, i.e., we first hypothesize that our approximation is totally accurate, then the top eigenvectors of Hessian should be the top eigenvector of $E[xx^T]$ Kronecker with the top eigenvectors of $E[M]$, and we design this method to test our hypothesis, and then show the figures. Besides, for the figures, I think we need more interpretations instead of letting the readers look at them directly. We can perhaps say ``We can see a diagonal pattern in Figure x, indicating that the $i$-th eigenvector of the layerwise Hessian indeed mainly comes from xxx''.} \ynote{There may be some differences because our explanation does not depend on the approximation is good for the E[M] part and we would like to present a more general model}

\subsection{Structure of Auto-correlation Matrix \texorpdfstring{$\E[\vx\vx^T]$}{ExxT}}
\label{sec:xxT}
From \cref{fig:xxT}, we can see $\E[\vx\vx^T]$ are all close to rank 1. This phenomenon is also observed along the training trajectory and in other networks.
\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxT_sigval_d20_MNIST_Exp1_FC2_fixlr0.01R1_E-1_fc1fc2.pdf}
        \caption{Fully connected layers of FC2 (MNIST)}
        \label{fig:xxT_sig_fc2}%
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxT_sigval_d20_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_fc1fc2.pdf}
        \caption{Fully connected layers of LeNet5 (CIFAR10)}
        \label{fig:xxT_sig_lenet}
    \end{subfigure}%
    \hfill
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/xxT/xxTConv_sigval_d20_CIFAR10_Exp1_LeNet5_fixlr0.01_E-1.pdf}
        \caption{Convolution layers of LeNet5 (CIFAR10)}
        \label{fig:xxT_sig_lenet}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspectrum of $\E[\vx\vx^T]$ for different layers in different models. All are close to rank 1.\znote{This figure should go to appendix as there is not much useful information which specifically requires a graph to visualize}}
    \label{fig:xxT}
\end{figure}

Let the $\hE[\vx]$ be normalized $\E[\vx]$ for FCs and the first left singular vector of $\E[\vx]$ for conv. We also find that the top eigenvector of $\E[\vx\vx^T]$ ($\vv_1$) is almost equal to $\hE[\vx]$, as their inner product are usually larger than 0.998. This suggests that $\E[\vx]\E[\vx]^T$ approximately equals to $\E[\vx\vx^T]$ and dominates the covariance $\mSigma_\vx$. It is verified as the Spectral norm of $\E[\vx]\E[\vx]^T$ is more than 5 times that of $\mSigma_\vx$ in all our experiments. This is natural because $\vx$ are output of ReLU layers and thus nonnegative, for all layers other than the input layer.
 \rnote{We should just show the empirical observation that the covariance matrix has small spectral norm, therefore by standard matrix perturbation bounds the true matrix is still close to rank 1 and the top eigenvector is close to $\E[x]$}

\subsection{Further Approximation for the Top Eigenspace of Layerwise Hessian}
\label{sec:approx_top_eig}
Since the top eigenvector of $\E[\vx\vx^T]$, $\vv_1$ is approximately $\hE[\vx]$, with results in \cref{sec:eigen_corr}, around $n$ top eigenvectors of layer-wise Hessian are all in $\Krsp(\hE[\vx])$. 

Let the number of top eigenvectors of layerwise Hessian are approximated in $\Krsp(\hE[\vx])$ be $s$. In most cases as in \cref{fig:Corr_fc} and \cref{fig:Corr_conv}, $s \approx n$. Thus, for $i \leq s$, $i$th eigenvector $\vh_i \approx \vu_i \otimes \hE[\vx]$ for some $\vu_i \in \R^n$. Thus, for any $k \leq s$, the top $k$ eigenspace of the Hessian can be approximated as $\mU_k \otimes \hE[\vx]$, where columns of $\mU_k$ are $\vu_1, \ldots, \vu_k$.

Note that this approximation and most explanations in \cref{sec:empirical} does not depend on $\vv_1 \approx \hE[\vx]$ and as we can substitute $\vv_1$ for $\hE[\vx]$. We use $\hE[\vx]$ to show the identity of $\vv_1$ in most cases and give more intuition for the discussion.

\cnote{I fell like we are using too many formulas and a bit complicated notations, which will confuse the readers. Here perhaps we need to remind people what is Krsp and what is n. I think it's better to interpret things by words instead of formulas in the main text since this is not really a theoretical paper. For example, for the last sentence in the above paragraph, we can instead say ``Thus, the top $s$ eigenvectors of the Hessian can be well approximated by the Kronecker products between $E[x]$ and the top eigenvectors of $E[M]$.'' I would assume that people can only remember what is $M$ and $xx^T$, so perhaps we need to avoid using notations like $u_i$ if possible. Also, I think the use of ``temporary variables'' is not necessary in most of the texts. We can use English instead, and it also saves some space I guess. I mean, instead of saying ``$\forall i\leq s$'', we can say ``for the first $s$ eigenvectors of ...''}

Also, for some FC layers, the eigenvector correspondance heatmap of $\E[\mM]$ has a diagonal pattern in the first $s$ columns, as shown in \cref{fig:Corr_fc}. We can further approximate the $\vu_i$'s as the $i$th eigenvector of $\E[\mM]$. In this case, $\mU_k$ is the top $k$ eigenspace of $\E[\mM]$. There are also some cases where $s$ is considerably smaller than $n$, and larger than $n$ in rare cases. We will discuss them in the Appendix.

==> Old_files/pac_bayes_old.tex <==
\label{sec:pac}

\rnote{For this section, you should first define PAC-Bayes bound and explain the role of prior and posterior. Then you should say what posterior \cite{dziugaite2017computing} optimize over and explain how our posterior is different. After that skip all the details about calculation and directly show the results (the table, the figures might also belong to appendix). This shouldn't be a very long section.}

\subsection{Methods}
\cnote{We need to briefly explain the PAC-Bayes bound in \citet{dziugaite2017computing}, e.g., what is SNN, what does the bound look like, what's prior/posterior.}
Our layer-wise Hessian approximation can be used to efficiently improve the computing of nonvacuous PAC-Bayes generalization bounds presented in \citet{dziugaite2017computing}.\ynote{Should we cite in () or in the sentence?}\cnote{In the sentence.} The core part of their algorithm is to model the posterior as a multivariate normal distribution $\N(\vw, \diag(\vs))$ and optimizing $\vw$ and $\vs$. Intuitively, the optimization of $\vs$ is to search for an optimal deviation of each parameter that can balance the the training error and the KL divergence between prior and posterior. Since the covariance matrix is diagonal, the search is along the direction of each standard basis. In general, the variance should be larger for a flatter direction and smaller for a sharper direction. However, directions of the standard basis may not be the optimal direction for the search. If we consider the loss landscape close to the minimum, sharper directions correspond to the Hessian's eigenvectors of lareger eigenvalues. \ynote{Cite or put some description in the Preliminary?} Thus, it may be a good idea to perform the search using the basis of Hessian's eigenvectors.

Since we can only use standard basis to calculate training loss, a change of basis is required. A direct change of basis using eigenvectors of Hessian is computationally prohbitive.\ynote{except for very small networks.} However, efficient approximate change of basis can be performed using the Kronecker factorized layer-wise Hessians. Let $\mU$ be the full eigenspace of $\E[\mM]$ and $\mV$ be that of $\E[\vx\vx^T]$ with eigenvectors as columns. We define $\Mat$ as the reshape of a vector to the shape of the parameter matrix $\mW$ of that layer. Then, let $\vv$ be the vector in standard basis. We have the new vector $\vv'$ in Hessian basis as
\begin{equation}
    \vv' = \vect\left[\mU^T\Mat(\vv)\mV\right].
\end{equation}
The calculation is thus much faster and a reverse process can be easily applied to change a vector back to the standard basis.\ynote{Should we omit the entire calculation? Or just say implicit matrix multiplication and refer to Appendix} This algorithm is called Approx Hessian.

In addition, since the posterior mean $\vw$ changes during the optimization, it is reasonable to use eigenvectors of the Hessian with respect to the current $\vw$. This algorithm is called Iterative Hessian, where we calculate new eigenvectors every several epochs.\ynote{We should results where we calculate new eigenvectors every 10 epochs but also tried other settings. Should we specify 10 here?}

\subsection{Results}
We used identical dataset, network structures and experiment settings as in \citet{dziugaite2017computing}, with a few adjustments in hyperparameters. We also adding FC2 we used in \cref{sec:hessian}. T-$600_{10}$ and FC$2_{10}$ are trained on standard MNIST while all others are trained on 2-class MNIST. The results are shown in \cref{tab:pac}. The network are expressed as X-$n^m$, indicating $m$ hidden layers with $n$ nodes each, trained on true labels (X=T) or random labels (X=R).\ynote{The generalization gap shown is our generalization gap, which is similar to the previous work.}

\begin{table}[th]
\caption{Optimized PAC-Bayes bound with Hessian Information \znote{need change}}

\begin{center}
\begin{tabular}{lccccccc}
\multicolumn{1}{c}{\bf Experiments}  & T-$600$ & T-$1200$ & T-$300^2$ & T-$600^2$ & R-$600$ & T-$600_{10}$ & FC$2_{10}$
\\ \hline \\
Generalization gap      & 0.0153  & 0.0161  & 0.0150 & 0.0148  & 0.4925 & 0.0180 & 0.0208 \\
Vanilla*                 & 0.1540  & 0.1754 &  0.1686 & 0.1921  & 0.6046  & 0.2879 & 0.4165 \\
Approx Hessian          & 0.1464 & 0.1726  & 0.1417  & 0.1712  & \textbf{0.5653} & 0.2424 & 0.2725 \\
Iterative Hessian       &  \textbf{0.1198}  & \textbf{0.1417}  & \textbf{0.1249}  & \textbf{0.1456}  & 0.5681 & \textbf{0.2132}   & \textbf{0.2145}  \\
\end{tabular}
\end{center}
\label{tab:pac}
\end{table}
\ynote{Iterative Hessian for FC2 is still runing. Previous results have some hyperparameter issues.}

Compared with previous work and vanilla algorithm, we can see a significant decrease of PAC-Bayes bound using Approximated Hessian algorithm and a further decrease using Iterative Hessian algorithm. Bounds for standard MNIST are not as good but still nonvacuous.

We also plotted the natural logarithm of final variance, $\vs$. The Figure 5.1 shown below is for (Approx Hessian of T-600) \znote{FC2}. The basis is ordered with decreasing eigenvalues. We can see that direction associated with larger eigenvalue has a smaller variance. This agrees with our presumption that top eigenvectors are aligned with sharper directions and should have smaller variance after optimization.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/PacBayes/FC2_10cls/sigma_post_compare_iter_Sigma_post_MNIST_Exp1FC2_fixlr0.01_fc1.weight.pdf}
    \captionsetup{justification=centering}
    \caption{Variance of optimized posterior. (first hidden layer of FC2, trained on MNIST)}
    \label{fig:PAC}
\end{figure}

Detailed algorithms and experiment settings are in \cref{sec:appendix_pac}.

==> graveyard.tex <==
\subsection{First structure notes}
\subsubsection{Overlap of different models}
\begin{itemize}
    \item High overlap of top eigenspace of different models
    \item The peak of the overlap for layerwise eigenspace happens at dimension $n$, where $n$ is the number of output channels for convolutional layers and the number of output neurons for FC layers.
    \item Assumptions: The reason is that the gram matrix of the input of the layer is close to rank 1. For FC layers, it has been shown that $\E[\vx \vx^T]$ is close to rank 1.
    \item For convolutional layers, we have also observed that $\E[\mX \mX]^T]$ is close to rank 1, where $X$ is a matrix transformed from the input according to the modular hessian paper.
    \item The connections are still unclear and require more investigations.
\end{itemize}

\subsubsection{Kronecker product decomposition of Hessians for FC layers}
\begin{itemize}
    \item For FC networks, we can then express the weight hessian block w.r.t. the $p$-th and $q$-th layer in the form of $$\mH_{\vw^{(p)}\vw^{(q)}} l = \mU^{(p)T}\mA\mU^{(q)} \otimes \vx^{(p)}\vx^{(q)T}.$$
    \item We focus on Hessians with respect to a single layer. For a fixed layer $p$ if there is no confusion, we write
    $$\mH_{\vw\vw} l = \nabla_\vw^2 l = \mM \otimes \vx\vx^T.$$
    \item Show the approximation is good for top eigenvalues and top eigenspace.
    \item Assumption: The approximation is actually for $\mG_0+\mG_1+\mG_2$ in the paper (or $\mG_0+\mG_1$).
    \item Similar hierarchy structure in $\mM$ and/or $\vx\vx^T$. We can probably tSNE to observe the clustering in $\mM$ and/or $\vx\vx^T$.
\end{itemize}

\subsubsection{Random Label}
\begin{itemize}
    \item The disappearance of the gap between top $C$ eigenvalues and the bulk for random labels.
    \item Experiment on whether the top $C^2$ eigenvalues still exist (i.e. seperation between $\mG_2$ and $\mG_3$.
    \item Observe the clustering in $\Delta$ in the paper and $\mM$.
    \item Explain why Kronecker decomposition is still a good decomposition.
\end{itemize}

\subsection{Structure of \texorpdfstring{\E[\mM]}{EM}}
\ynote{Probably need more analysis on why the approximate is good.}

\snote{Clustering analysis on $\Delta$ matrices, maybe some provable claims on the initialization?
Observations for random label cases and corresponding explainations.}

\subsection{Structure of Output Hessian \texorpdfstring{$\E[\mM]$}{EM}}
\label{sec:struct_M}
\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/UTAU/UTAU_sigval_d30_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1_fc1fc2.pdf}
        \caption{Minimum}
        \label{fig:UTAU_spec_minima}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/UTAU/UTAU_sigval_d30_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E0_fc1fc2.pdf}
        \caption{Random Initialization}
        \label{fig:UTAU_spec_init}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenspectrum/UTAU/UTAU_sigval_d30_CIFAR10_RandomLabel_LeNet5_fixlr0.01_RLR1_E-1_fc1fc2.pdf}
        \caption{Minimum (Random Label)}
        \label{fig:UTAU_spec_RL}
    \end{subfigure}
    \captionsetup{justification=centering}
    \caption{Eigenspace overlap between models}
    \label{fig:UTAU_spec}
\end{figure}

\cref{fig:UTAU_spec_minima} and \cref{fig:UTAU_spec_init} shows the eigenspectrum of $\E[\mM]$ for FC2 networks at minimum and at initialization. In both cases we can see there are 9 or 10 outliers in the eigenspectrum. This phenomenon does not appear for dataset with random labels as shown in \cref{fig:UTAU_spec_RL}. Similar results are observed for other networks.

Gaps in eigenvalue distribution around dimension 10 are also observed in the eigenspectrum of full Hessians, agreeing with previous empirical studies. \citet{sagun2017empirical} suggests that there is a gap in Hessian eigenvalue distribution around the number of classes $C$ in most cases, where $C=10$ in our case. We conjecture this phenomenon is closely related to the structure of $\E[\mM]$ and will discuss more in \cref{sec:emp_outlier}.

\citet{papyan2019measurements} provides explanation for the gap in eigenspectrum using class clustering. Although we reproduced their results on their networks, there is no clear class clustering for both $\E[M]$ and layerwise Hessian at the Minimum for networks we experiment on. The reason is unclear but we conjecture that class clustering is only significant for very large networks.

The outliers at initialization, however, is easy to explain. Similar to \citet{papyan2019measurements} suggests for full Hessian, we observe logit clustering in $\E[\mM]$'s. Since there are $C$ logits, we would expect there are $C$ outliers. The results are shown in Appendix.

\subsection{Explanation for eigenspace overlap}
Moreover, since the neurons can be permuted to give equivalent models while changing eigenvectors, we can assume that eigenvectors of $\E[\mM]_1$ and $\E[\mM]_2$ have no correlation and thus have an expected inner product of $\frac{1}{\sqrt{n}}$. Thus, $\Overlap(\mV_1, \mV_2) =\frac{1}{k}\|\mV_1^T\mV_2\|^2_F = \frac{k}{n}$ and the overlap of top $k$ eigenspace of the true Hessian would be approximately $\frac{k}{n}(\hE[\vx]_1 \cdot \hE[\vx]_2)^2$. \ynote{Any further evidence/proof required?} In addition, for the first layer, models with the same dataset would have the same $\hE[\vx]$, and that would lead to an overlap close to 1 at dimension $n$.

Then, consider the $(n+1)$-th eigenvector of the first model $\vv_1$, since the top $n$ eigenvectors already span the full subspace $\mI_n \otimes \hE[\vx]_1$, $\vv_1$ will be orthogonal to this subspace. If $\hE[\vx]_1 \cdot \hE[\vx]_2$ is large, as we will shown empirically, $\vv_1$ will also be approximately orthogonal to $\mI_n \otimes \hE[\vx]_2$. The same applies to the $(n+1)$-th eigenvector of the second model, $\vv_2$. Then, again due to neuron permutation, we expect that $\vv_1 \cdot \vv_2$ is small. Thus, the overlap of the dimension $(n+1)$ eigenspace will decrease immediately and we will see a peak at dimension $n$. \ynote{Can there be a better/shorter explanation or just omit the explanation for the peak at dimension $n$?}

Indeed, we observe this phenomenon in () as shown in Fig. 4.4. In addition, the peak at dimension $n$ is high for all the layers. This would suggest that for all layers, $\hE[\vx]$ are similar for different models.

For layers where not all top $n$ eigenvectors can be approximated as Kronecker products of $\hE[\vx]$, we can observe a lower peak at dimension around $n$. This can be put into a more general model stated in Appendix.

We also observe similar overlap for convolutional layers and the peak dimension is the number of output channels. We do not have an explanation for this but it can be closely related to the case of FC layers. (see Appendix)

\subsection{Zero-mean Batch Normalization}
\snote{The approximation worsen, but is still relevant. Reason of low overlap: low correlation between $x$ in different layers, random permutation of neurons in FC layers.}

In order to further verify our conjecture that the good approximation and high overlap of top eigenspace both depend on the fact that $\E[\vx]\E[\vx]^T$ dominates $\mSigma_\vx$, we experiment on networks with zero-mean normalization where we subtract the mean of its inputs from them so $\E[\vx]$ become 0. In our experiments, it is carried out within a single batch and we use a large batch size in order to make the mean of each batch approximately the same. Thus, we have $\E[\vx] \approx 0$ for all the layers after this process. Note that the input data is also normalized.

Figure 4.5.1 shows the eigenspectrum of $\E[\vx\vx^T]$ after zero-mean normalization. As expected, the huge gap between the first and the second eigenvalue disappear. Also, the top eigenvector is no longer $\hE[x]$ as their overlap is ().

Thus, following our analysis in \cref{sec:xxT}, we would not be able to approximate the top $n$ eigenvectors as the Kronecker products of $\tx$. In this case, the approximation of the top eigenspace would be less accurate. This is shown in Figure 4.5.2.

In addition, the overlap of top $k$ eigenspace between different models can no longer be approximated as in \cref{eqn:model_overlap}. This would lead to a much lower overlap of top $k$ eigenspace for $k < n$ and a disappearance of the peak at dimension $n$, as shown in Figure 4.5.3.

\subsection{Further Approximation for the Top Eigenspace of Layerwise Hessian}
\label{sec:approx_top_eig}
Since the top eigenvector of $\E[\vx\vx^T]$, $\vv_1$ is approximately $\hE[\vx]$, with results in \cref{sec:eigen_corr}, around $n$ top eigenvectors of layer-wise Hessian are all in $\Krsp(\hE[\vx])$. 

Let the number of top eigenvectors of layerwise Hessian are approximated in $\Krsp(\hE[\vx])$ be $s$. In most cases as in \cref{fig:Corr_fc} and \cref{fig:Corr_conv}, $s \approx m$. Thus, for $i \leq s$, $i$th eigenvector $\vh_i \approx \vu_i \otimes \hE[\vx]$ for some $\vu_i \in \R^n$. Thus, for any $k \leq s$, the top $k$ eigenspace of the Hessian can be approximated as $\mU_k \otimes \hE[\vx]$, where columns of $\mU_k$ are $\vu_1, \ldots, \vu_k$.

Note that this approximation and most explanations in \cref{sec:empirical} does not depend on $\vv_1 \approx \hE[\vx]$ and as we can substitute $\vv_1$ for $\hE[\vx]$. We use $\hE[\vx]$ to show the identity of $\vv_1$ in most cases and give more intuition for the discussion.

\cnote{I fell like we are using too many formulas and a bit complicated notations, which will confuse the readers. Here perhaps we need to remind people what is Krsp and what is n. I think it's better to interpret things by words instead of formulas in the main text since this is not really a theoretical paper. For example, for the last sentence in the above paragraph, we can instead say ``Thus, the top $s$ eigenvectors of the Hessian can be well approximated by the Kronecker products between $E[x]$ and the top eigenvectors of $E[M]$.'' I would assume that people can only remember what is $M$ and $xx^T$, so perhaps we need to avoid using notations like $u_i$ if possible. Also, I think the use of ``temporary variables'' is not necessary in most of the texts. We can use English instead, and it also saves some space I guess. I mean, instead of saying ``$\forall i\leq s$'', we can say ``for the first $s$ eigenvectors of ...''}

Also, for some FC layers, the eigenvector correspondance heatmap of $\E[\mM]$ has a diagonal pattern in the first $s$ columns, as shown in \cref{fig:Corr_fc}. We can further approximate the $\vu_i$'s as the $i$th eigenvector of $\E[\mM]$. In this case, $\mU_k$ is the top $k$ eigenspace of $\E[\mM]$. There are also some cases where $s$ is considerably smaller than $m$, and larger than $m$ in rare cases. We will discuss them in the Appendix.

==> old_intro.tex <==
\label{sec:intro}
%Despite a lot of recent research, understanding the optimization and generalization for neural networks remain challenging problems: why can simple algorithm such as stochastic gradient descent optimize the complicated nonconvex objective, and why would the result generalize to unseen data? A common conjecture is that both problems are related to the loss landscape of neural networks. In this paper, we focus on an important aspect of the loss landscape \--- the layer-wise Hessian for neural networks along its training trajectory.

Neural network objectives are complicated and non-convex. However, in practice neural networks can be trained by simple algorithms and they perform well on test data. A common explanation is that neural network objectives have good loss landscapes for optimization and generalization. In this paper we study the structure of Hessians for neural network objectives.

Hessians capture important properties of the loss landscape. For optimization, Hessian information is used explicitly in second order optimization algorithms, and even for gradient-based algorithms properties of the Hessian are often leveraged in analysis \citep{sra2012optimization}. For generalization, the Hessian captures the local structure of the loss function near a local minimum, which is believed to be related to generalization gaps \citep{keskar2016large}. %which is related to the intuition of flat vs. sharp local minimum, and can be incorporated into generalization bounds using ideas like PAC-Bayes bounds.

What structures are there in the Hessian of neural network objectives?
Previous works \citep{sagun2017empirical, papyan2018full} observed that the Hessian often has around $c$ large eigenvalues, where $c$ is the number of classes. In this paper we find more structure in the top eigenvectors and eigenspace of layer-wise Hessian. We can explain such structures by approximating the Hessian using a Kronecker decomposition. Our new understanding of the Hessian can be directly used to improve explicit generalization bounds similar to those in \citet{dziugaite2017computing}.

%We show that the eigenspaces of layer-wise Hessians also have other surprising behaviors: the top eigenspace of layer-wise Hessians from two randomly trained models have a high overlap at a dimension that is approximately equal to the layer's output-width; when the top eigenvectors of the layer-wise are viewed as matrices (with the same dimensions as the weight matrix), such matrices are approximately rank 1.

%We show that under a decoupling conjecture, one can approximate the layer-wise Hessian using the Kronecker product of the covariance of its input and its output Hessian. This Kronecker decomposition and the low rank properties of its two components allow us to explain the interesting properties of the layer-wise Hessians. Our explanation also shows that when batch normalization is enabled some of these properties no longer holds. 

%Better understanding of the Hessian can give more insights into optimization and generalization. As a directly application of our results, we show that the Hessian structure can be used to improve the PAC-Bayes bound computed in \citet{}; we also show that the general structure of the Hessian suggests a simple way of incorporating second-order information in optimization without large overhead.

%\rnote{Maybe make the above three paragraph even shorter?}

\subsection{Our Results}
\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.6\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=0.49\textwidth]{Figures/SubspaceOverlap/NLeNet5_multi_hyperparam/DimOverlap_CIFAR10_LeNet5_normnew_fixlr0.001_X_LeNet5_normnew_fixlr0.01_X_LeNet5_normnew_fixlr0.01_momentum_fc1.pdf}
        \includegraphics[width=0.49\textwidth]{Figures/SubspaceOverlap/NLeNet5_multi_hyperparam/DimOverlap_CIFAR10_LeNet5_normnew_fixlr0.001_X_LeNet5_normnew_fixlr0.01_X_LeNet5_normnew_fixlr0.01_momentum_conv1.pdf}
        \caption{Overlap between dominate eigenspace of layer-wise Hessian at different minima for fc1:LeNet5 (\textbf{left}) with output dimension 120 and conv1:LeNet5 (\textbf{right}) with output dimension 6.}
        \label{fig:intro_overlap}
    \end{subfigure}%
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{Figures/Eigenvec_single/Top_Eigenvector_sigs_CIFAR10_Exp1_LeNet5_fixlr0.01R1_E-1fc1.pdf}
        \caption{Top singular values of the top 4 eigenvectors of the layer-wise Hessian of fc1:LeNet5 after reshaped as matrix.}
        \label{fig:intro_lowrank}
    \end{subfigure}
    \caption{Some surprising observations on the structure of layer-wise Hessians.}
    \label{fig:intro_figs}
\end{figure}
\textbf{Structure of Hessians:} Consider two neural networks trained with different random initializations and potentially different hyper-parameters; their weights are usually nearly orthogonal. One might expect that the top eigenspace of their layer-wise Hessians are also very different. However, this is surprisingly false: the top eigenspace of the layer-wise Hessians have a very high overlap, and the overlap peaks at the dimension of the layer's output (see \cref{fig:intro_overlap}).
Another interesting phenomenon is that if we express the top eigenvectors of a layer-wise Hessian as a matrix with the same dimensions as the weight matrix, then the matrix is approximately rank 1. In \cref{fig:intro_lowrank} we show the singular values of several such reshaped eigenvectors. 

\textbf{Kronecker Factorization:} We show that both of these new properties of Hessians can be explained by a Kronecker Factorization approximation. Under a decoupling conjecture, we can approximate the layer-wise Hessian using the Kronecker product of the output Hessian and input auto-correlation. This Kronecker approximation directly implies that the eigenvectors of the layer-wise Hessian should be approximately rank 1 when viewed as a matrix. We also analyze the behavior of the two components: the auto-correlation of the input is often very close to a rank 1 matrix and the output Hessian often has around $c$ large eigenvectors. We show that when the input auto-correlation component is approximately rank 1, the layer-wise Hessians indeed have high overlap at the dimension of the layer's output, and the spectrum of the layer-wise Hessian is similar to the spectrum of the output Hessian. On the contrary, when the model is trained with batch normalization, the input auto-correlation matrix is much farther from rank 1 and the layer-wise Hessian often does not have the same low rank structure.

%\textbf{Leveraging Hessian Structure:}
%Better understanding of the Hessian can give more insights into optimization and generalization. 
As a direct application of our results, we show that the Hessian structure can be used to improve the PAC-Bayes bound computed in \citet{dziugaite2017computing}. %; we also show that the general structure of the Hessian suggests a simple way of incorporating second-order information in optimization without large overhead.



==> projection_optimization.tex <==
\znote{May want to cite \citet{ghorbani2019investigation}}

To further understand the optimization process, we conducted a grid search of different optimization schemes by varying the step sizes and network depth, as well as comparing between traditional batch normalization and projection off E[x]. Models optimized by projecting off of E[x] were generally found to converge to full training accuracy with fewer steps than models trained with normal SGD. In fact, for most step sizes $>$ 0.01, both shallow and deep fully connected networks trained with the projection method converged in even fewer steps than when trained with batch normalization. Additionally, the optimal step size for the projection method is greater than the optimal step size for normally trained models as well as BN-trained models for shallow networks. As network depth increases, variation in convergence speed also increases so it is more difficult to make conclusive generalizations, but it can be observed that the optimal projection step size grows closer to that of the control and BN-trained models. However, when compared to batch normalization, the performance of projection-trained models is less stable against varying learning rates. Additionally, batch normalization leads to slightly improved generalization over the projection method, although both models perform better than normally trained FC6 networks on test data. On the smaller FC3 network, projection tends to result in slightly worse test performance than the control models.

\begin{figure}[th]
    \centering
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{fig/proj_bn_learningCurves.png}
        \caption{TBD}
        \label{fig:overlap_approx}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.49\textwidth}
        \centering
        \captionsetup{justification=centering}
        \includegraphics[width=\textwidth]{fig/proj_convergence_speeds.png}
        \caption{TBD}
        \label{fig:eigenval_approx}
    \end{subfigure}
    \caption{TBD}
    \label{fig:three graphs}
\end{figure}


==> templete.tex <==
\section{Submission of conference papers to ICLR 2021}

ICLR requires electronic submissions, processed by
\url{https://openreview.net/}. See ICLR's website for more instructions.

If your paper is ultimately accepted, the statement {\tt
  {\textbackslash}iclrfinalcopy} should be inserted to adjust the
format to the camera ready requirements.

The format for the submissions is a variant of the NeurIPS format.
Please read carefully the instructions below, and follow them
faithfully.

\subsection{Style}

Papers to be submitted to ICLR 2021 must be prepared according to the
instructions presented here.

%% Please note that we have introduced automatic line number generation
%% into the style file for \LaTeXe. This is to help reviewers
%% refer to specific lines of the paper when they make their comments. Please do
%% NOT refer to these line numbers in your paper as they will be removed from the
%% style file for the final version of accepted papers.

Authors are required to use the ICLR \LaTeX{} style files obtainable at the
ICLR website. Please make sure you use the current files and
not previous versions. Tweaking the style files may be grounds for rejection.

\subsection{Retrieval of style files}

The style files for ICLR and other conference information are available online at:
\begin{center}
   \url{http://www.iclr.cc/}
\end{center}
The file \verb+iclr2021_conference.pdf+ contains these
instructions and illustrates the
various formatting requirements your ICLR paper must satisfy.
Submissions must be made using \LaTeX{} and the style files
\verb+iclr2021_conference.sty+ and \verb+iclr2021_conference.bst+ (to be used with \LaTeX{}2e). The file
\verb+iclr2021_conference.tex+ may be used as a ``shell'' for writing your paper. All you
have to do is replace the author, title, abstract, and text of the paper with
your own.

The formatting instructions contained in these style files are summarized in
sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.

\section{General formatting instructions}
\label{gen_inst}

The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).
Use 10~point type with a vertical spacing of 11~points. Times New Roman is the
preferred typeface throughout. Paragraphs are separated by 1/2~line space,
with no indentation.

Paper title is 17~point, in small caps and left-aligned.
All pages should start at 1~inch (6~picas) from the top of the page.

Authors' names are
set in boldface, and each name is placed above its corresponding
address. The lead author's name is to be listed first, and
the co-authors' names are set to follow. Authors sharing the
same address can be on the same line.

Please pay special attention to the instructions in section \ref{others}
regarding figures, tables, acknowledgments, and references.


There will be a strict upper limit of 8 pages for the main text of the initial submission, with unlimited additional pages for citations. Note that the upper page limit differs from last year!Authors may use as many pages of appendices (after the bibliography) as they wish, but reviewers are not required to read these. During the rebuttal phase and for the camera ready version, authors are allowed one additional page for the main text, for a strict upper limit of 9 pages.

\section{Headings: first level}
\label{headings}

First level headings are in small caps,
flush left and in point size 12. One line space before the first level
heading and 1/2~line space after the first level heading.

\subsection{Headings: second level}

Second level headings are in small caps,
flush left and in point size 10. One line space before the second level
heading and 1/2~line space after the second level heading.

\subsubsection{Headings: third level}

Third level headings are in small caps,
flush left and in point size 10. One line space before the third level
heading and 1/2~line space after the third level heading.

\section{Citations, figures, tables, references}
\label{others}

These instructions apply to everyone, regardless of the formatter being used.

\subsection{Citations within the text}

Citations within the text should be based on the \texttt{natbib} package
and include the authors' last names and year (with the ``et~al.'' construct
for more than two authors). When the authors or the publication are
included in the sentence, the citation should not be in parenthesis using \verb|\citet{}| (as
in ``See \citet{Hinton06} for more information.''). Otherwise, the citation
should be in parenthesis using \verb|\citep{}| (as in ``Deep learning shows promise to make progress
towards AI~\citep{Bengio+chapter2007}.'').

The corresponding references are to be listed in alphabetical order of
authors, in the \textsc{References} section. As to the format of the
references themselves, any style is acceptable as long as it is used
consistently.

\subsection{Footnotes}

Indicate footnotes with a number\footnote{Sample of the first footnote} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches
(12~picas).\footnote{Sample of the second footnote}

\subsection{Figures}

All artwork must be neat, clean, and legible. Lines should be dark
enough for purposes of reproduction; art work should not be
hand-drawn. The figure number and caption always appear after the
figure. Place one line space before the figure caption, and one line
space after the figure. The figure caption is lower case (except for
first word and proper nouns); figures are numbered consecutively.

Make sure the figure caption does not get separated from the figure.
Leave sufficient space to avoid splitting the figure and figure caption.

You may use color figures.
However, it is best for the
figure captions and the paper body to make sense if the paper is printed
either in black/white or in color.
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
\end{center}
\caption{Sample figure caption.}
\end{figure}

\subsection{Tables}

All tables must be centered, neat, clean and legible. Do not use hand-drawn
tables. The table number and title always appear before the table. See
Table~\ref{sample-table}.

Place one line space before the table title, one line space after the table
title, and one line space after the table. The table title must be lower case
(except for first word and proper nouns); tables are numbered consecutively.

\begin{table}[t]
\caption{Sample table title}
\label{sample-table}
\begin{center}
\begin{tabular}{ll}
\multicolumn{1}{c}{\bf PART}  &\multicolumn{1}{c}{\bf DESCRIPTION}
\\ \hline \\
Dendrite         &Input terminal \\
Axon             &Output terminal \\
Soma             &Cell body (contains cell nucleus) \\
\end{tabular}
\end{center}
\end{table}

\section{Default Notation}

In an attempt to encourage standardized notation, we have included the
notation file from the textbook, \textit{Deep Learning}
\cite{goodfellow2016deep} available at
\url{https://github.com/goodfeli/dlbook_notation/}.  Use of this style
is not required and can be disabled by commenting out
\texttt{math\_commands.tex}.


\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}



\section{Final instructions}
Do not change any aspects of the formatting parameters in the style files.
In particular, do not modify the width or length of the rectangle the text
should fit into, and do not change font sizes (except perhaps in the
\textsc{References} section; see below). Please note that pages should be
numbered.

\section{Preparing PostScript or PDF files}

Please prepare PostScript or PDF files with paper size ``US Letter'', and
not, for example, ``A4''. The -t
letter option on dvips will produce US Letter files.

Consider directly generating PDF files using \verb+pdflatex+
(especially if you are a MiKTeX user).
PDF figures must be substituted for EPS figures, however.

Otherwise, please generate your PostScript and PDF files with the following commands:
\begin{verbatim}
dvips mypaper.dvi -t letter -Ppdf -G0 -o mypaper.ps
ps2pdf mypaper.ps mypaper.pdf
\end{verbatim}

\subsection{Margins in LaTeX}

Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+
from the graphicx package. Always specify the figure width as a multiple of
the line width as in the example below using .eps graphics
\begin{verbatim}
   \usepackage[dvips]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.eps}
\end{verbatim}
or % Apr 2009 addition
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
for .pdf graphics.
See section~4.4 in the graphics bundle documentation (\url{http://www.ctan.org/tex-archive/macros/latex/required/graphics/grfguide.ps})

A number of width problems arise when LaTeX cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command.
